Personalized Academic Research Paper Recommendation System

A huge number of academic papers are coming out from a lot of conferences and journals these days. In these circumstances, most researchers rely on key-based search or browsing through proceedings of top conferences and journals to find their related work. To ease this difficulty, we propose a Personalized Academic Research Paper Recommendation System, which recommends related articles, for each researcher, that may be interesting to her/him. In this paper, we first introduce our web crawler to retrieve research papers from the web. Then, we define similarity between two research papers based on the text similarity between them. Finally, we propose our recommender system developed using collaborative filtering methods. Our evaluation results demonstrate that our system recommends good quality research papers.

==> goal.tex <==
\section{Research Goals}

Our proposed system consists of the following components: data
crawler, text similarity measurer, recommender, and user interface.
In this section, we will describe detailed plan for developing each
component.

\subsection{Data Crawler}
For our paper recommendation system, we need
a huge number of papers to provide to the system as inputs. The
first component data gatherer crawls data of papers from the web.
The data of papers include title, author(s), keywords, and abstract.
Our first goal is to build data crawlers for IEEE Xplorer and ACM
Digital Library, given an URL for a conference page on that site. As
these sites do not provide programming APIs, we have no choice but
to crawl the web page directly and analyze their HTML pages. We are
going to get the data of papers from three different research areas
(Machine Learning, Databases, Human-Computer Interaction) in
computer science. Basically, papers from top conferences of each
area will be gathered. For example, papers from VLDB, SIGMOD and
ICDE for Databases area will be included. Our gatherer will store
the gathered data into a set of files and the data will be retrieved
by our recommender system.

\subsection{Text Similarity Measurer}
When the gathered data are given to the system, we are ready to
build a model. In other words, we need to figure out each user's
preference as well as each paper's feature based on the gathered
data. As our raw data consists of large amount of texts, extracting
and modeling paper (item) features requires natural language
processing. Especially, we need to calculate how each document is
similar in the sense of topic. User preference is also modeled based
on the analysis of their own papers. For this task, we
referred~\cite{manning:ir}, describing language models for
information retrieval (chapter 12) and text classification based on
Na?ve Bayes model (chapter 13). We built a Bag-of-words model,
detailed in the next section.

\subsection{Recommender}
The core part of this system is recommender, finding out papers
which the target user may like. For this part, we implemented
several collaborative filtering methods. According to recent surveys
~\cite{su:survey,adomavicius:survey}, collaborative filtering (CF)
methods are classified into two groups: memory-based and
model-based. With memory-based methods, we load all the data into
the memory during training process like lazy classifiers. When a
request is given, we find similar users or items to the queried user
or item, and generate items to recommend. This approach is simple
and easy to implement, but not so much scalable. On the other hand,
model-based methods build a model to generalize given training data.
It does not have the whole data in memory, so scalability is much
better compared to memory-based methods.~\cite{breese:empirical}
Recently, matrix factorization approaches~\cite{manning:ir} are
known as the most efficient and accurate, especially after those
approaches won the Netflix prize in 2009.

In our system, we were about to build memory-based methods,
including user-based~\cite{breese:empirical} (seeking similar users
first, and recommend their favorite items) and
item-based~\cite{sarwar:item} (looking for similar items first, and
rate based on their average rating) memory-based models. Also, we
were thinking of building matrix factorization with singular value
decomposition (SVD) as well. However, due to the innate
characteristics in our data (discussed in Section 3), we adopted
only a simple Naive Recommender and item-based
CF.~\cite{sarwar:item}

\subsection{User Interface}
To show the result of our recommender system, we
will implement a simple Graphical User Interface for users.
Basically, our GUI is, when a user search for a researcher on our
GUI, to suggest a list of papers which might be interesting to the
researcher. Therefore, our GUI will contain functions in order to
search a list of papers for a particular researcher. This part is
not done up to this point, according to our schedule.

